Enhancing Prostate Cancer Diagnosis with Deep Learning: A Study using mpMRI Segmentation and Classification

Prostate cancer (PCa) is a severe disease among men globally. It is important to identify PCa early and make a precise diagnosis for effective treatment. For PCa diagnosis, Multi-parametric magnetic resonance imaging (mpMRI) emerged as an invaluable imaging modality that offers a precise anatomical view of the prostate gland and its tissue structure. Deep learning (DL) models can enhance existing clinical systems and improve patient care by locating regions of interest for physicians. Recently, DL techniques have been employed to develop a pipeline for segmenting and classifying different cancer types. These studies show that DL can be used to increase diagnostic precision and give objective results without variability. This work uses well-known DL models for the classification and segmentation of mpMRI images to detect PCa. Our implementation involves four pipelines; Semantic DeepSegNet with ResNet50, DeepSegNet with recurrent neural network (RNN), U-Net with RNN, and U-Net with a long short-term memory (LSTM). Each segmentation model is paired with a different classifier to evaluate the performance using different metrics. The results of our experiments show that the pipeline that uses the combination of U-Net and the LSTM model outperforms all other combinations, excelling in both segmentation and classification tasks.

==> old_relatedwork.tex <==
\section{Related Work}\label{sec:related}
The use of DL technologies in healthcare has led to the development of predictive systems for PCa diagnosis. mpMRI images are a popular modality in this regard due to their non-invasive collection method~\cite{mehta2021computer}. For better patient care, mpMRI and DL combined in automated CAD systems can save doctors' time and lead to rapid PCa diagnosis~\cite{gavade2023automated}. 

Litjens \etal~\cite{litjens2014computer} proposed a two-stage CAD system utilizing MRI images for screening, yielding a sensitivity of 69\% and a specificity of 83\%. In the first stage, they performed voxel feature extraction and later used candidate regions to obtain cancer likelihood. 
Likewise, Artan \etal~\cite{artan2010prostate} introduced a CAD system for PCa localization on multi-spectral MRI, demonstrating commendable sensitivity and specificity for cancer detection and an average Dice similarity coefficient (DSC) of 0.82.
Peng \etal~\cite{peng2013quantitative} developed a CAD system for PCa detection and differentiation from normal tissue using mpMRI, achieving an impressive Area Under the Curve (AUC) of 0.85 for distinguishing cancer from normal tissue.
Brosch \etal~\cite{brosch2018deep} devised a DL approach for boundary detection using neural networks and segmentation of the prostate in MRI images. Their method demonstrated impressive results, achieving a DSC of 0.89 and a mean absolute distance of 1.4 mm. 
Liu \etal~\cite{liu2009prostate} proposed a method for PCa segmentation using MRI, achieving an average DSC of 0.815 for segmenting the prostate region and 0.666 for segmenting the cancerous regions.


Among approaches utilizing DNN, Tian \etal~\cite{tian2018psnet} proposed PSNet for MRI prostate segmentation, achieving an average DSC of 0.94 and an average Hausdorff distance of 4.16 mm on the test dataset.  
Aldoj \etal~\cite{aldoj2020automatic} employed a DenseNet-like U-net architecture to achieve automatic prostate zonal segmentation from MRI images, obtaining an impressive overall DSC of 0.92 in their limited dataset. They utilized cost-sensitive support vector machines and conditional random fields to refine segmentation. 
Karimi \etal~\cite{karimi2018prostate} introduced a custom DNN architecture for prostate segmentation, employing a training strategy based on statistical shape models, resulting in a commendable average DSC of 0.895. 
Abraham \etal~\cite{abraham2019automated} utilized a VGG16 DNN with an ordinal classifier to evaluate Gleason Score (GS) for PCa grading, achieving accurate grade prediction and reducing the mortality rate due to PCa. 
Cao \etal~\cite{cao2019joint} proposed FocalNet, a multiclass DNN for the simultaneous detection of PCa lesions and prediction of their aggressiveness using GS, contributing to the development of automated clinical decision support systems for PCa diagnosis. 
% Duran \etal~\cite{duran2022prostattention} proposed ProstAttention-Net, a deep attention model for the segmentation of PCa by aggressiveness in MRI scans, achieving a DSC of 0.69 and micro-precisions of 0.88 and 0.83 for high-risk and intermediate-risk cancer classification, 
% respectively, outperforming other reference segmentation models such as U-Net, DeepLabv3+, and E-Net.

Benefiting from transfer learning, Zhong \etal~\cite{zhong2019deep} proposed a model for classifying PCa in mpMRI. Their approach showed promise in improving the accuracy and efficiency of PCa diagnosis, providing valuable clinical decision support to radiologists.  Mehta \etal~\cite{mehta2021computer} developed a patient-level classification framework for PCa diagnosis using mpMRI and clinical features. Their system achieved an AUC of 0.89 for distinguishing cancer from benign tissue and AUC values of 0.79 and 0.85 for differentiating low-grade and high-grade cancer, respectively. 
Combining textural and morphological analysis, Zhang \etal~\cite{zhang2021new} proposed a new approach for diagnosing PCa using MRI, achieving an overall accuracy of 89.6\%, a sensitivity of 87.5\%, and specificity of 90.8\%. This approach shows promise in improving the accuracy and efficiency of PCa diagnosis, providing valuable clinical decision support for radiologists. 
% Mahapatra and Buhmann ~\cite{mahapatra2016visual} developed an active learning-based method for prostate MRI segmentation using visual saliency cues. Their approach incorporates principles from visual saliency to query labels of informative samples, improving the efficiency and accuracy of prostate segmentation from MRI. 
Recently, Sun \etal~\cite{sun2023deep} developed DL models for detecting and localizing clinically significant PCa in mpMRI. 
% Hasan \etal~\cite{hasan2023breast} developed a highly automated and efficient algorithm for extracting deep features. This algorithm effectively utilizes T2W-TSE and STIR MRI sequences to differentiate between pathological and healthy breast MRI scans. 
Gavade \etal~\cite{segnet} introduced DeepSegNet and trained in CT images to perform semantic segmentation. Later, Gavade \etal~\cite{gavade_peripheral} highlighted the promise of data-driven algorithms in PCa analysis through mpMRI. They pinpointed nnU-Net's promising performance in precisely segmenting PCa across the peripheral zone and central gland regions. Interestingly, ResNet-50 emerged as the frontrunner in classification, showcasing remarkable accuracy. These findings underscore the transformative potential of transfer learning for DL methodologies.

% , showcasing their capacity to enhance precision and streamline the 
By leveraging state-of-the-art DL models and developing new pipelines on mpMRI data, the emerging research can potentially revolutionize PCa diagnosis. Integrating AI-driven analyses with conventional clinical assessments will ultimately lead to improved diagnostic and treatment planning processes for PCa using mpMRI.
